Weighted Model Counting in the two variable fragment with Cardinality Constraints: A Closed Form Formula

Weighted First-Order Model Counting (WFOMC) computes the weighted sum of the models of a first-order theory on a given finite domain. WFOMC has emerged as a fundamental tool for probabilistic inference. Algorithms for WFOMC that run in polynomial time w.r.t. the domain size are called lifted inference algorithms. Such algorithms have been developed for multiple extensions of FO2(the fragment of first-order logic with two variables) for the special case of symmetric weight functions. We introduce the concept of lifted interpretations as a tool for formulating polynomials for WFOMC. Using lifted interpretations, we reconstruct the closed-form formula for polynomial-time FOMC in the universal fragment of FO2, earlier proposed by Beame et al. We then expand this closed-form to incorporate existential quantifiers and cardinality constraints without losing domain-liftability. Finally, we show that the obtained closed-form motivates a natural definition of a family of weight functions strictly larger than symmetric weight functions.

==> counting.tex <==
\section{FOMC for Counting Quantifiers}
\emph{Counting quantifiers} are expressions of the form
$\exists x^{\geq m}y.\Phi$, $\exists^{\leq m}y.\Phi$, and
$\exists^{= m}y.\Phi$. The extension of FO$^2$ with such quantifiers
is denoted as C$^2$ \cite{COUNTING_REF}.  In this section, we show how
FOMC in C$^2$ can be performed by exploiting the formula for FOMC in
FO$^2$ with cardinality constraints. We assume that the counting
quantifier $\exists^{\leq m}y.\Phi$ is expanded to
$\bigvee_{k=0}^m\exists^{=m}y.\Phi$, and the expressions
$\exists^{\geq m}y.\Phi$ is first transformed to
$\neg(\exists^{\leq m-1}y.\Phi)$ and then expanded. We are therefore
left with quantifiers of the form $\exists^{=m}y.\Phi$.  The easy case
is when $\Phi$ contains only one free variable i.e.,
$\exists^{=m}x.\Phi(x)$.  In this case, this sub-formula is replaced
with $A(x)$, where $A$ is a new unary predicate, and conjuncted with
$\forall x(A(x)\leftrightarrow\Phi(x))$ and the cardinality constraint
$\card{A}\ =m$. It is easy to see that the FOMC of the expanded
formula with the new cardinality constraint is equal to the FOMC of
the original formula.  The case in which $\Phi$ contains both free
variables $x$ and $y$ deserves more attention. W.l.o.g, we can assume
that $\Phi(x,y)$ is the atomic formula $R(x,y)$. We will present a
transformation for FOMC of
$(A(x) \leftrightarrow \exists^{=m}yR(x,y))$. We will then show that
such a transformation can be used to handle arbitrary case of FOMC
with counting quantifiers.

\begin{lemma}
    \label{lem:counting-quantifiers}
    Let $C$ be a domain of $n$ elements, let $m$ be $0 < m < n$ and let
    $A$ be a new unary predicate, and $f_1,\dots, f_m$,
    be $m$ new binary predicates. 
    For every assignment $\omega$ 
    that satisfies $\forall x.(A(x)\leftrightarrow \exists^{=m}y.
    R(x,y)))$, 
    there are $m!^{\card{A^\omega}}$ extensions of $\omega$  
    that satisfy the following formulas, where $A^\omega = \{c\in
    C\mid\omega(A(c))=1\}$. 
    \begin{align}
    \label{eq:exists-k-encoding-1}
    & \forall x.\left(A(x) \rightarrow  \forall y.\left(R(x,y)\leftrightarrow
                                     \bigvee_{i=1}^mf_i(x,y)\right)\right)\\ 
    \label{eq:exists-k-encoding-2}
    & \bigwedge_{i\neq j=1}^m\forall xy.\left(f_i(x,y) \rightarrow \neg
                                     f_j(x,y) \right) \\ 
    \label{eq:exists-k-encoding-3}
    & \forall x.A(x)\rightarrow \bigwedge_{i=1}^m\exists y.f_i(x,y) \\ 
    \label{eq:exists-k-encoding-4}
    & \bigwedge_{i=1}^m\left(\card{f_i} = \card{A}\right) \\
    \label{eq:exists-k-encoding-5}
    & \maximize(A,f_1,\dots,f_m)
    \end{align}
    Viceversa: if $\omega$ is an assignment that satisfies
    \eqref{eq:exists-k-encoding-1}-\eqref{eq:exists-k-encoding-5},
    it also satisfies $\forall x.(A(x)\leftrightarrow\exists^{=m}y.R(x,y))$.
\end{lemma}
\begin{arxiv}    
Before proving the lemma we
prove the following preliminary result
\begin{proposition}
 \label{prop:lem-counting-quantif}
        If $\omega\models\mbox{\eqref{eq:exists-k-encoding-1}--\eqref{eq:exists-k-encoding-4}}$
        and $c\in A^\omega$, then $c$ has exactly $m$ $R$-successors.
\end{proposition}
\begin{proof}
  If $c\in A^\omega$ then by axioms
    \eqref{eq:exists-k-encoding-3} there are $m$ domain elements $c_1,\dots,c_m$ 
    such that $(c,c_i)\in f_i(x,y)^\omega$. Axiom \eqref{eq:exists-k-encoding-2}
    guarantees that all the $c_i$'s are distinct.  By axiom
    \eqref{eq:exists-k-encoding-4} we have that if $(c,c_i)\in f_i(x,y)^\omega$ and $(c,c_i')\in f_i(x,y)^\omega$, then $c_i=c_i'$.
     Finally, axiom
    \eqref{eq:exists-k-encoding-1} guarantees that 
    $(c,d)\in R^\omega$ iff $(c,d)\in\cup_if_i^\omega$, i.e., if
    $d=c_i$ for some $i$, 
    which proves that $c$ has exactly $m$ $R$-successors.  
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:counting-quantifiers}]
  Suppose that
  $\omega\models\forall x(A(x)\leftrightarrow\exists^{=m}y,R(x,y))$.
  For every $c\in A^{\omega}$, let $c_1,\dots,c_m$ be an enumeration
  of the $m$ $R$-successors of $c$ in $\omega$. Notice that there are $m!$
  such an enumerations.\\
  Let us extend $\omega$ to $f_i$ such that
  $f_i^\omega=\{(c,c_i)\mid c\in A^{\omega}\}$. Since for every
    $c\in A^\omega$ there are $m!$ distinct extensions, then in
    total we have $(m!)^{\card{A^\omega}}$ possible choices.  We
  have that the axioms
  \eqref{eq:exists-k-encoding-2}-\eqref{eq:exists-k-encoding-4} are
  satisfied by construction. To check axiom
    \eqref{eq:exists-k-encoding-1}, suppose that $c\in A^\omega$
    (if $c\not\in A^{\omega}$ the axiom is trivially satisfied),
    then $c$ has $m$ $R$-successors by hypothesis and by construction
    they are all in $\{c'\in C\mid (c,c')\in f_i^\omega,1\leq i\leq m\}$ which guarantees
    that axiom \eqref{eq:exists-k-encoding-1} holds.  Finally, we have
    to prove that $\omega\models\maximize(A,f_1,\dots,f_m)$.  Let
    $\omega'$ be an interpretation that agree with $\omega$ on all the
    predicates but $A,f_1,\dots,f_m$ such that
    $\omega'\models\mbox{\eqref{eq:exists-k-encoding-1}--\eqref{eq:exists-k-encoding-4}}$;
    Suppose, by contradiction, that
    $(\card{A^\omega}, \card{f_1^\omega},\dots, \card{f_m^\omega})
    \prec (\card{A^{\omega'}}, \card{f_1^{\omega'}},\dots,
    \card{f_m^{\omega'}})$; Axiom 
    \eqref{eq:exists-k-encoding-4} implies that
    $\card{A^{\omega'}} =
    \card{f_1^{\omega'}}=\dots=\card{f_m^{\omega'}}$.  This implies that
    $\card{A^{\omega'}} > \card{A^\omega}$; Therefore there is a
    $d\in A^{\omega'}$ which is not in $A^\omega$. By 
    Proposition~\ref{prop:lem-counting-quantif},
    $d$ has $m$ R-successors, while in $\omega$, $d$ does
    not have $m$ $R$-successors. This means that $\omega$ and
    $\omega'$ do not agree on the interpretation of $R$ which
    contradicts the hypothesis that $\omega$ and $\omega'$ agree on
    the interpretations of all the predicate but $A$ and $f_i$. 

    Viceversa, let us prove that
  $\omega\models\mbox{\eqref{eq:exists-k-encoding-1}--\eqref{eq:exists-k-encoding-5}}$
  implies
  $\omega\models\forall x(A(x)\leftrightarrow\exists^{=m}y.R(x,y))$.  If
  $\omega\models A(c)$ then, by Proposition~\ref{prop:lem-counting-quantif}, $c$ has
  exactly $m$ $R$-successors and therefore
  $\omega\models\exists^{=m}y.R(c,y)$.  If $\omega\models\exists^{=m}y.R(c,y)$ then
  since $\omega\models\maximize(A,f_1,\dots,f_n)$ implies that
  $\omega\models A(c)$. 
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:counting-quantifiers}]
  \color{blue}
  Suppose that
  $\omega\models\forall x(A(x)\leftrightarrow\exists^{=m}y,R(x,y))$.
  For every $c\in A^{\omega}$, let $c_1,\dots,c_m$ be an enumeration
  of the $m$ $R$-successors of $c$ in $\omega$. Notice that there are $m!$
  such an enumerations.\\
  Let us extend $\omega$ to $f_i$ such that
  $f_i^\omega=\{(c,c_i)\mid c\in A^{\omega}\}$. Since for every
    $c\in A^\omega$ there are $m!$ distinct extensions, then in
    total we have $(m!)^{\card{A^\omega}}$ possible choices.  We
  have that the axioms
  \eqref{eq:exists-k-encoding-2}-\eqref{eq:exists-k-encoding-4} are
  satisfied by construction. To check axiom
    \eqref{eq:exists-k-encoding-1}, suppose that $c\in A^\omega$
    (if $c\not\in A^{\omega}$ the axiom is trivially satisfied),
    then $c$ has $m$ $R$-successors by hypothesis and by construction
    they are all in $\{c'\in C\mid (c,c')\in f_i^\omega,1\leq i\leq m\}$ which guarantees
    that axiom \eqref{eq:exists-k-encoding-1} holds.  Finally, we have
    to prove that $\omega\models\maximize(A,f_1,\dots,f_m)$.  Let
    $\omega'$ be an interpretation that agree with $\omega$ on cardinalities of  all the
    predicates but $A,f_1,\dots,f_m$ such that
    $\omega'\models\mbox{\eqref{eq:exists-k-encoding-1}--\eqref{eq:exists-k-encoding-4}}$;
    Suppose, by contradiction, that
    $(\card{A^\omega}, \card{f_1^\omega},\dots, \card{f_m^\omega})
    \prec (\card{A^{\omega'}}, \card{f_1^{\omega'}},\dots,
    \card{f_m^{\omega'}})$; Axiom 
    \eqref{eq:exists-k-encoding-4} implies that
    $\card{A^{\omega'}} =
    \card{f_1^{\omega'}}=\dots=\card{f_m^{\omega'}}$.  This implies that
    $\card{A^{\omega'}} > \card{A^\omega}$; Therefore, $A^{\omega'}$ has atleast one more constant than $A^\omega$.
    By Proposition~\ref{prop:lem-counting-quantif},
    each such constant in $A^{\omega'}$ has $m$ R-successors, meaning that the cardinality of $R$ in $\omega'$ is larger than in $\omega$. This means that $\omega$ and
    $\omega'$ do not agree on the cardinality of interpretation of $R$ which
    contradicts the hypothesis that $\omega$ and $\omega'$ agree on
    the cardinality of all the predicate but $A$ and $f_i$. 

    Viceversa, let us prove that
  $\omega\models\mbox{\eqref{eq:exists-k-encoding-1}--\eqref{eq:exists-k-encoding-5}}$
  implies
  $\omega\models\forall x(A(x)\leftrightarrow\exists^{=m}y.R(x,y))$.  If
  $\omega\models A(c)$ then, by Proposition~\ref{prop:lem-counting-quantif}, $c$ has
  exactly $m$ $R$-successors and therefore
  $\omega\models\exists^{=m}y.R(c,y)$.  If $\omega\models\exists^{=m}y.R(c,y)$ then
  since $\omega\models\maximize(A,f_1,\dots,f_n)$ implies that
  $\omega\models A(c)$. 
\end{proof}


Lemma~\ref{lem:counting-quantifiers} can be generalized for
multiple counting quantifiers.
\begin{lemma}
    \label{lem:multiple-counting-quantifiers}
    Let $C$ be a domain of $n$ elements, let $0 < m_1,\dots,m_k < n$
    be $k$ integers. For every $i$ let $A_i$ 
   be a new unary predicate, and $f_{i1},\dots, f_{im_i}$,
    be $m_i$ new binary predicates. 
    For every assignment $\omega$ 
    that satisfies $\bigwedge_{i=1}^k\forall x.(A_i(x)\leftrightarrow \exists^{=m_i}y.
    R_i(x,y)))$, 
    there are $\prod_{i=1}^km_i!^{\card{A_i^\omega}}$ extensions
    of $\omega$, that satisfy axioms 
    \eqref{eq:exists-k-encoding-1}--\eqref{eq:exists-k-encoding-5},
    where $A$, $f_j$ and $R$ are replaced with $A_i$, $f_{ij}$ and
    $R_i$ (we call these axioms the $i$-version of
    \eqref{eq:exists-k-encoding-1}--\eqref{eq:exists-k-encoding-5})
    for every $1\leq i \leq k$. 
    Viceversa: if $\omega$ is an assignment that satisfies
    all the $i$-th versions of 
    \eqref{eq:exists-k-encoding-1}-\eqref{eq:exists-k-encoding-5},
    it also satisfies $\forall
      x.(A_i(x)\leftrightarrow\exists^{=m_i}y.R_i(x,y))$.
\end{lemma}
\begin{proof}
  The proof is a straightforward generalization of the proof of
  lemma~\ref{lem:counting-quantifiers}, where $A$, $f_j$ and $R$ are
  replaced with their indexed version $A_i$, $f_{ij}$ and $R_i$.
  Notice that $\omega$ is required to satisfy multiple maximization
  constraints, however they are all independent, and they can be
  maximized separately. 
\end{proof}

The above Lemma allows us to replace all the counting quantified predicates like 
  $\exists^{=m_i}y.R_i(x,y)$  with a new
  unary predicate $A_{i}$ and associated relational predicates
  $f_{i1}(x,y), \dots , f_{im_i}(x,y)$. The result of this
  substitution in conjunction with the additional axioms
  \eqref{eq:exists-k-encoding-1}-\eqref{eq:exists-k-encoding-5}, will
  result in a FO$^2$ formula with cardinality constraints and $k$
  maximization axioms $\maximize(\{A_{i},f_{ij}\})$. 
\end{arxiv}
  
\begin{theorem}
\label{thm:counting-quantifiers}
Let $\Phi$ be a C$^2$ formula containing $k$ occurrences of
sub-formulas of the form $\exists^{=m_i}y.R_i(x,y)$ for $1\leq
i\leq k$. Let $\Phi'$ be the
formula obtained by replacing each of such occurrence with $A_{i}(x)$
for a new predicate $A_i$ conjuncted with the $i$-th version of 
\eqref{eq:exists-k-encoding-1}-\eqref{eq:exists-k-encoding-4}
 for each $1\leq i\leq k$. Then, 
$\fomc(\Phi,n)$ is equal to 
  \begin{align}
  \label{eq:counting-quantifiers-begin}
    \sum\limits_{\substack{
                              \bk,\bh  \\
                              (\bk,\bh)\models |A_i|=|f_{ij}| \\
                              (\bk,\bh)\models\maximize(\{A_i,f_{i1},\dots,f_{im_i}\})}}
    \hspace{-3em}\frac{(-1)^{\sum_{l}\bk(P_l)}F(\bk,\bh,\{n_{ijv}\})}{\prod_{i=1}^k(m_i!)^{\bk(A_{i})}}
  \end{align}
  where $\{P_l\}$ are the unary auxillary predicates introduced to deal with existential quantifiers %
   \footnote{In the rest of the paper, we assume $(-1)^{\sum_{l}\bk(P_l)}$ factor to be implicit in $F(\bk,\bh,\{n_{ijv}\})$  }. 
% with
%   \begin{align*}
% F(\bk,\bh,\{n_{ijv}\})=
% \binom{n}{\bk}\prod_{0\leq i\leq j \leq 2^u-1}
%                      \binom{\bk(i,j)}{\bh^{ij}} \prod_{0\leq v\leq 2^b-1}n_{ijv}^{h^{ij}_v}
% \end{align*}
\end{theorem}

\begin{proof}
If $\omega$ is an assignment that satisfies $\Phi$ then by
lemma~\ref{lem:multiple-counting-quantifiers}, it can be extended in
$\prod_{i=1}^k(m_i!)^{\card{A_i^\omega}}$ different assignments that
satisfy
\begin{align}
  \label{eq:phi-prime-and-counting-quantif}
  \Phi'\wedge\bigwedge_{i=1}^k\left(\left(\card{f_{ij}}=\card{A_i}\right)\wedge\maximize(\{A_i,f_{i1},\dots,f_{im_i})\}_{i=1}^k\right)
\end{align}
Viceversa if $\omega'$ is an assignment satisfying
\eqref{eq:phi-prime-and-counting-quantif} then it is an extension of
an assignment that satisfies $\Phi$. 
Notice that different $\omega$ generate different extensions. 
Furthermore for every $(\kh)$ on the extended langauge, 
if $\omega_1$ and $\omega_2$ are two assignments that satisfy $\Phi$ such that 
$\card{R_{i}^{\omega_1}}=\card{R_{i}^{\omega_2}}=(\kh)(R_i)$, then they both generate
$\prod_{i=1}^k(m_i!)^{\bk(A_i)}$ extensions that satisfy
\eqref{eq:phi-prime-and-counting-quantif}. This means that 
for every $(\kh)$ the number of assignments that satisfy $\Phi$ can be
obtained by deviding the assignments that satisfy
\eqref{eq:phi-prime-and-counting-quantif} by 
$\prod_{i=1}^k(m_i!)^{\bk(A_i)}$. 
 \end{proof}


\begin{arxiv} 
\begin{example}
  Consider the formula $\Phi=\forall x(\forall y \neg R(x,y) \vee
  \exists^{=2}R_2(x,y))$. i.e., every object has either no $R$
  successor or two $R$-successors. 

  
\begin{align*}
   &\fomc(\Phi,n)  = \sum\limits_{\substack{\kh \\
                              \bk(A)=(\kh)(f_1)=(\kh)(f_2) \\
  (\kh)\models\maximize(A,f_1,f_2)}}
  \frac1{2^{\bk(A)}} \times \\
&{n\choose \bm k}(-1)^{\bk(P_1) + \bk(P_2)}\prod_{0\leq i\leq j\leq
  2^6-1}{\bk(i,j) \choose \bh^{ij}}\prod_{0\leq v\leq 2^6-1}n_{ijv}^{h^{ij}_v}
\end{align*}
where $n_{ijv}$ is $0$ or $1$ depending on wether the corresponding lifted
interpretation $\tau_{ijv}$ satisfies $\Phi(\{x,y\})$ where
$\Phi(x,y)$ is the following pure universal formula: 
\begin{align}
\label{eq:phi1}
& \neg R(x,y)\vee A(x) \ \wedge \\
\label{eq:phi2}
& A(x) \rightarrow (R(x,y)\leftrightarrow f_1(x,y)\vee f_2(x,y)) \ \wedge \\
\label{eq:phi3}
& f_1(x,y) \rightarrow \neg f_2(x,y)\ \wedge  \\
\label{eq:phi4}
& P_1(x) \rightarrow \neg (A(x) \rightarrow f_1(x,y))\ \wedge  \\
\label{eq:phi5}
& P_2(x) \rightarrow \neg (A(x) \rightarrow f_2(x,y))
\end{align}
To cope with the counting quantifier $\exists^{=2}y.R(x,y)$ we have
introduced the new unary predicate $A(x)$ and two new binary predicates
$f_1(x,y)$ and $f_2(x,y)$. 
\eqref{eq:phi1} is the result of replacing $\exists^{=2}y.
R(x,y)$ with $A(x)$ in $\Phi$; \eqref{eq:phi2} and 
\eqref{eq:phi3} are the instances of axioms
\eqref{eq:exists-k-encoding-1} and 
\eqref{eq:exists-k-encoding-2}; 
\eqref{eq:phi4} and \eqref{eq:phi5} is the result of the
transformation of \eqref{eq:exists-k-encoding-3} that removes
existential quantifiers on $f_1(x,y)$ and $f_2(x,y)$ by introducing two new unary predicates
$P_1(x)$ and $P_2(x)$. 
Finally, in order to take into account the cardinality restriction and
the maximization constraint, in the summation we consider only the $\kh$ that
satisfy $\bk(A)=(\kh)(f_1)=(\kh)(f_2)$ and maximize
$\left<\bk(A),(\kh)(f_1),(\kh)(f_2)\right>$. 
\end{example}
\end{arxiv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "template"
%%% End:

